Data-driven stochastic spectral modeling for coarsening of the two-dimensional Euler equations on the sphere

A resolution-independent data-driven stochastic parametrization method for subgrid-scale processes in coarsened fluid descriptions is proposed. The method enables the inclusion of high-fidelity data into the coarsened flow model, thereby enabling accurate simulations also with the coarser representation. The small-scale parametrization is introduced at the level of the Fourier coefficients of the coarsened numerical solution. It is designed to reproduce the kinetic energy spectra observed in high-fidelity data of the same system. The approach is based on a control feedback term reminiscent of continuous data assimilation. The method relies solely on the availability of high-fidelity data from a statistically steady state. No assumptions are made regarding the adopted discretization method or the selected coarser resolution. The performance of the method is assessed for the two-dimensional Euler equations on the sphere. Applying the method at two significantly coarser resolutions yields good results for the mean and variance of the Fourier coefficients. Stable and accurate large-scale dynamics can be simulated over long integration times.

==> 2023-04-24 Arxiv/figures_paper/unused_text.tex <==
We consider four types of forcing in our coarse numerical simulations, all of which are based on the mean-reverting forcing presented in Eqs. \eqref{eq:spectral_forcing}-\eqref{eq:forced_equations}. The forcing types are the following: \begin{enumerate}
    \item The forcing as presented in \eqref{eq:general_forcing} and included in the equations following \eqref{eq:forced_equations}, referred to as \textit{continuous forcing}.
    \item The forcing \eqref{eq:general_forcing}, computed after completing a time step. That is, $W_{n+1}$ is obtained from the unforced system, after which a correction term $hF$ is added to the vorticity field. Note that $F$ is determined from $W_{n+1}$ in this setting. We refer to this as \textit{nudging}.
    \item The forcing $F_P:=\Pi_P^\perp F$, where $F$ follows from \eqref{eq:general_forcing}. This projection leads to a forcing that can be written as \begin{equation}
        \dot{W} = [P, W] + [P, Z], \label{eq:energy_preserving_forcing}
    \end{equation} 
    where $[P, Z] = F_P$. The formulation \eqref{eq:energy_preserving_forcing} preserves the kinetic energy and is referred to as \textit{energy-preserving forcing.}
    \item The forcing $F_W: = \Pi_W^\perp F$, where $F$ follows from \eqref{eq:general_forcing}. Using this projection the forcing can be written as \begin{equation}
        \dot{W} = [P, W] + [Q, W],
    \end{equation} where $[Q, W] = F_W$. This type of forcing preserves the Casimir functions and is referred to as \textit{Casimir-preserving forcing}. 
\end{enumerate}
The Casimir-preserving forcing alters the velocity which advects the vorticity and can therefore be regarded as a Leray-type regularization model \cite{leray1934mouvement}. For stochastic forcing terms, one recovers the stochastic advection by Lie transport (SALT) \cite{holm2015variational} method for the two-dimensional Euler equations, which has been the subject of recent studies \cite{cotter2019numerically, ephrati2022datadriven}.

The energy-preserving property of the last type of forcing can be proved directly from the definition of the Hamiltonian. Using that the inverse Laplacian is a symmetric operator, i.e., $(\Delta_N^{-1}A) B = A (\Delta_N^{-1}B)$, conservation of the Hamiltonian readily follows.

==> figures_paper/unused_text.tex <==
We consider four types of forcing in our coarse numerical simulations, all of which are based on the mean-reverting forcing presented in Eqs. \eqref{eq:spectral_forcing}-\eqref{eq:forced_equations}. The forcing types are the following: \begin{enumerate}
    \item The forcing as presented in \eqref{eq:general_forcing} and included in the equations following \eqref{eq:forced_equations}, referred to as \textit{continuous forcing}.
    \item The forcing \eqref{eq:general_forcing}, computed after completing a time step. That is, $W_{n+1}$ is obtained from the unforced system, after which a correction term $hF$ is added to the vorticity field. Note that $F$ is determined from $W_{n+1}$ in this setting. We refer to this as \textit{nudging}.
    \item The forcing $F_P:=\Pi_P^\perp F$, where $F$ follows from \eqref{eq:general_forcing}. This projection leads to a forcing that can be written as \begin{equation}
        \dot{W} = [P, W] + [P, Z], \label{eq:energy_preserving_forcing}
    \end{equation} 
    where $[P, Z] = F_P$. The formulation \eqref{eq:energy_preserving_forcing} preserves the kinetic energy and is referred to as \textit{energy-preserving forcing.}
    \item The forcing $F_W: = \Pi_W^\perp F$, where $F$ follows from \eqref{eq:general_forcing}. Using this projection the forcing can be written as \begin{equation}
        \dot{W} = [P, W] + [Q, W],
    \end{equation} where $[Q, W] = F_W$. This type of forcing preserves the Casimir functions and is referred to as \textit{Casimir-preserving forcing}. 
\end{enumerate}
The Casimir-preserving forcing alters the velocity which advects the vorticity and can therefore be regarded as a Leray-type regularization model \cite{leray1934mouvement}. For stochastic forcing terms, one recovers the stochastic advection by Lie transport (SALT) \cite{holm2015variational} method for the two-dimensional Euler equations, which has been the subject of recent studies \cite{cotter2019numerically, ephrati2022datadriven}.

The energy-preserving property of the last type of forcing can be proved directly from the definition of the Hamiltonian. Using that the inverse Laplacian is a symmetric operator, i.e., $(\Delta_N^{-1}A) B = A (\Delta_N^{-1}B)$, conservation of the Hamiltonian readily follows.
